Learning to combine primitive skills: A step towards versatile robotic manipulation

Manipulation tasks such as preparing a meal or assembling furniture remain highly challenging for robotics and vision. Traditional task and motion planning (TAMP) methods can solve complex tasks but require full state observability and are not adapted to dynamic scene changes. Recent learning methods can operate directly on visual inputs but typically require many demonstrations and/or task-specific reward engineering. In this work we aim to overcome previous limitations and propose a reinforcement learning (RL) approach to task planning that learns to combine primitive skills. First, compared to previous learning methods, our approach requires neither intermediate rewards nor complete task demonstrations during training. Second, we demonstrate the versatility of our vision-based task planning in challenging settings with temporary occlusions and dynamic scene changes. Third, we propose an efficient training of basic skills from few synthetic demonstrations by exploring recent CNN architectures and data augmentation. Notably, while all of our policies are learned on visual inputs in simulated environments, we demonstrate the successful transfer and high success rates when applying such policies to manipulation tasks on a real UR5 robotic arm.

==> figures/hrlbc_envs.tex <==
\begin{figure*}
\mbox{} \vspace{-.5cm}\\
\centering
  \begin{subfigure}[t]{0.7\textwidth}
     \includegraphics[width=0.45\textwidth]{imgs/UR5-Bowl-Sim.png}
   \includegraphics[width=0.45\textwidth]{imgs/UR5-Bowl-Real.png}
   \caption{UR5-Bowl }
     \label{fig:ur5_bowl}
  \end{subfigure}
 \begin{subfigure}[t]{0.7\textwidth}
 \includegraphics[width=0.45\textwidth]{imgs/UR5-Salad-Sim.png}
   \includegraphics[width=0.45\textwidth]{imgs/UR5-Salad-Real.png}
   \caption{UR5-Breakfast }
     \label{fig:ur5_breakfast}
  \end{subfigure}\hfill
  \\ \mbox{} \vspace{-.1cm}\\
  \caption{Two complex manipulation tasks with a single success reward used for the RLBC experiments: (a)~task of bringing the cube to the bowl, (b)~task of pouring the cup and the bottle into the bowl. (Left) simulation, (right) real. \todo{update real robot images with the ones from the video} \vspace{-.3cm} }
\label{fig:hrlbc_tasks}
\end{figure*}


==> figures/teaser.tex <==
\begin{figure}
\centering
%trim=left bottom right top, clip
\includegraphics[trim=80 0 150 0, clip, width=\linewidth]{imgs/teaser_breakfast.pdf}
%\includegraphics[width=0.9\linewidth]{imgs/teaser_salad.png}
\caption{A vocabulary of primitive robotics skills learned with behavioral cloning is combined 
%with the reinforcement learning policy 
to successfully perform a more complex task in our UR5-Breakfast environment.\vspace{-.1cm}}
\label{fig:teaser}
\end{figure}


==> figures/timeline.tex <==
\begin{figure}[t]
\centering
 %trim=left bottom right top, clip
 %\includegraphics[trim=0 70 0 50, clip, width=0.9\linewidth]{imgs/timeline.pdf}
 \includegraphics[trim=0 70 0 50, clip, width=0.9\linewidth]{imgs/timeline.pdf}
 \vspace{-.2cm}
\caption{Temporal hierarchy of master and skill policies.\vspace{-.1cm}}
\label{fig:timeline}
\end{figure}

==> tables/bcrl_breakfast.tex <==
\begin{table}
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{lcccc}
\toprule
\begin{tabular}[c]{@{}c@{}}UR5-Breakfast \\ scenario\end{tabular} & \begin{tabular}[c]{@{}c@{}}BC-ordered \\ (simulated)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RLBC \\ (simulated)\end{tabular} & \begin{tabular}[c]{@{}c@{}}BC-ordered \\ (real)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RLBC \\ (real)\end{tabular} \\
\midrule
% UR5-Bowl &  100\% & 100\% & 17/20 & \textbf{20/20} \\
% \midrule
Simple &  91\% & \textbf{93\%} & 16/20 & 16/20 \\
Hard & 43\% & \textbf{82\%} & 8/20 & \textbf{16/20}\\
\bottomrule
\end{tabular}
\caption{Comparison of RLBC and manually ordered BC skills on simple and hard scenarios of the UR5-Breakfast task.\vspace{-.8cm}}
\label{tab:hrlbc_real}
\end{table}
